Hierarchical Multi Agent DRL for Soft Handovers Between Edge Clouds in Open RAN

Multi-connectivity (MC) for aerial users via a set of ground access points offers the potential for highly reliable communication. Within an open radio access network (O-RAN) architecture, edge clouds (ECs) enable MC with low latency for users within their coverage area. However, ensuring seamless service continuity for transitional users-those moving between the coverage areas of neighboring ECs-poses challenges due to centralized processing demands. To address this, we formulate a problem facilitating soft handovers between ECs, ensuring seamless transitions while maintaining service continuity for all users. We propose a hierarchical multi-agent reinforcement learning (HMARL) algorithm to dynamically determine the optimal functional split configuration for transitional and non-transitional users. Simulation results show that the proposed approach outperforms the conventional functional split in terms of the percentage of users maintaining service continuity, with at most 4% optimality gap. Additionally, HMARL achieves better scalability compared to the static baselines.

==> old.tex <==
\section{Introduction}
%Due to the evolution of service-critical application, new classes of services yielding highly constrained requirements have been arising in the latest years. Examples of these classes of service are Highly Reliable Low Latency communications, having latency requirement on the range of tens of milliseconds and reliability requirements that can accept error rates as low as $1e{-4}$. Serving users that deploy these services and complying with their requirements can be challenging, more so if the users are also roaming in the network. In fact, as users disconnect from one base station and connect to a new one they employ a break-and-reconnect strategy \cite{wang2016handover}, taking from 5 to 10 ms for the transition, making it hard to guarantee the compliance to upper-cited constraints. To avoid breaking and recreating connections while roaming, the infrastructure can employ CoMP Joint Transmission to serve the users using multiple base stations (BSs) at a time. Finally, to comply with the delay requirements H-CRAN can benefit from the use of Functional Split (FS), enabling the deployment of the network functions needed from signal processing up to the user data processing at different computing premises in the network. In H-CRAN those premises take the names "Edge Clouds" (ECs) and Central Cloud (CC), where ECs take care of the computing for a subset of the existing BSs (called domain), and the CC can host functions coming from the different ECs and connects the infrastructure to the core network. Depending on the function placement (called split), functions can be hosted either at ECs or CC, but the split choice can highly impact the resources of the HCRAN infrastructure, leading to interesting trade-offs between QoS for the users and resource consumption of different parts of the infrastructure. Finally, the whole scenario is affected by the existence of users that can cross between different EC domains (transitional users), that have to be handled by multiple ECs at the same time and require an higher degree of centralization to benefit from CoMP.

%The evolution of mission-critical applications created new classes of services yielding highly constrained requirements (e.g. latency and reliability). Complying with those constraints becomes increasingly challenging as the users begin to roam in the network, such as in the case of aerial hosts, making multi-connectivity and seamless handover between access points paramount to the fulfillment of the service requirements. 

Aerial users performing mission-critical applications have high reliability and strict latency requirements. Complying with such requirements becomes increasingly challenging as roaming users move from one location to another, since handover procedures necessitate the simultaneous termination and establishment of multiple connections with different access points. Multi-connectivity avoids the latter problem, having users connected to multiple access points at a time, allowing for a soft-handover, i.e., avoiding service interruption during handovers, at the cost of higher resources usage. Open Radio Access Network (O-RAN) architecture allows for multi-connectivity via the centralization of processing functions related to base stations (O-RAN Radio Units, O-RU) \cite{bassoy2017coordinated} at the premises of O-RAN Distributed Units (O-DUs) if involved O-RUs are part of the same coverage area, or at O-RAN Centralized Unit (O-CU) otherwise.
%. While such centralization can be performed at O-DUs for O-RUs under the same O-DU coverage area, processing has to be moved to the O-CU in the case of O-RUs belonging to different O-DUs' coverage areas.  
To enable such centralization, it is possible to employ functional split \cite{larsen2018survey}, 
%Functional split enables decoupling of hardware and software in O-RAN, thanks to which the chain of functions needed to process one O-RU and its users' data can be split into two sub-chains, dividing the computation of such sub-chains between O-DUs and O-CU. 
 moving processing functions to the O-CU when higher centralization means are needed for the multi-connectivity of transitional users (i.e., users connected 
to O-RUs belonging to different coverage areas).  
Functional split affects the network in multiple ways: from the delay experienced by users to the infrastructure resources usage (i.e., the load on O-DUs and bandwidth usage). In particular, multi-connectivity for transitional users impacts infrastructure's resources heavily, due to higher centralization needed and multiple O-DUs handling them at a time. 

In this paper, we focus on enabling soft handovers for transitional users, while ensuring compliance with the service requirements of all users and network resource utilization. To accomplish this, a Hierarchical Multi-Agent Reinforcement Learning (HMARL) algorithm is employed to take  function split 
decisions in order to maximize users' service continuity (complying with users' service's reliability requirements), focusing particularly on transitional users. 

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.45]{img/split.pdf}
    \caption{Functional Split representation and resource consumption tradeoffs.}
    \label{fig:schema}
\end{figure}

\

\section{System Model and Problem Formulation}

In this paper, we employ the Hybrid Cloud Radio Access Networks (H-CRAN) architecture. H-CRAN is composed of a single O-CU, called Central Cloud (CC) connected to multiple O-DUs called Edge Clouds (ECs) via the midhaul interface (O-RAN's F1 interface). Every EC is connected to several O-RUs, forming a coverage area.
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.7]{img/hcran.pdf}
    \caption{H-CRAN infrastructure with the aerial user moving from one EC (green coverage area) to another (blue coverage area), becoming transitional (purple shade) when connected to different ECs' O-RUs. }
    \label{fig:hcran}
\end{figure}
More information about the infrastructure used can be found in \cite{delay}. The processing functions required to handle cells and users in the network can be split between ECs and CC premises thanks to functional splitting, with split choices heavily impacting the resource utilization of the infrastructure (ECs' and midhaul link's loads), as depicted in Figure \ref{fig:schema} \cite{wang2017centralize}.
O-RUs serving a user must deploy the same functional split in order to enable multi-connectivity, with the splits being restricted to split $1$ to $3$ when handling transitional users using multi-connectivity.
%due to the higher degree of centralization needed. 
In this study, we propose to deploy two sets of functions: one for transitional users, i.e., $F_t$, and one for the users moving within the coverage area of one EC (non-transitional users), i.e., $F_{nt}$.
%For realism purposes, each EC deploys two different function chains: one for transitional users, $F_t$, and one for the users roaming inside their domain (non-transitional users), $F_{nt}$. Users move in the system following stochastic differential equations \cite{smith2022flexible} and deploy a service $k$ yielding a certain E2E Delay threshold $D_{th}^k$ and a reliability error threshold $\varepsilon^k$. 
Users movements are modeled as stochastic differential equations \cite{smith2022flexible}. Each user deploys a service $k$ requiring a certain end-to-end (E2E)  delay threshold to be respected, i.e., $D_{th}^k$, and a reliability error threshold $\varepsilon^k$  as the quality of service (QoS). Given the delay experienced by a user $D_u$, the reliability is modeled as the probability of complying with the delay threshold of service $k$ \cite{salehi2023reliability} with the latter constraint satisfied when:
    
%deploy a service $k$ yielding a certain E2E Delay threshold $D_{th}^k$, a reliability error threshold $\varepsilon^k$. Finally, we considered two finite resources whose consumption threshold cannot be exceeded at any point in time: the Giga Operations Per Second of any EC and the total bandwidth consumption of the link between ECs and CC, the midhaul bandwidth (respectively $G_{th}$ and ${BW}_{mid,th}^\tau$). The way the decisions about split interplays with the latter resources' usage can be seen in Figure \ref{fig:schema}, where choosing higher splits translates to higher load on the ECs, eventually nullifying the midhaul load and vice-versa. The values of the GOPS used and the midhaul bandwidth load generated at time $\tau$ by any EC (respectively $G_e^\tau$ and ${BW}_{mid,e}^\tau$) can be expressed using pre-computed reference values as described in \cite{wang2017centralize}. Given the delay experienced by a user $D_u$ e model the reliability as the probability of complying with the delay threshold of service $k$  as seen in \cite{salehi2023reliability} and the latter constrain is respected when  
\begin{equation}
    P(D_u > D^k_{th}) < \varepsilon^k.
\end{equation}

Our aim is to maximize the number of users achieving service continuity, so we define $R(U)$ as the ratio of users whose reliability requirement is satisfied within the set of users $U$:
\begin{equation}
    R(U) = \frac{1}{|U|} \sum_{u}^U\mathbbm{1}(P(D_u > D^k_{th}) < \varepsilon^k).
\end{equation}

Finally, given $T$ as the set of transitional users, $E$ as the set of ECs, $BW_{mid,th}$ and $G_{th}$ as the maximum load on the midhaul link in terms of bandwidth used and the maximum load of Giga Operation Per Second (GOPS) on any EC, respectively, we model our objective function as: 
\begin{subequations}
\begin{equation}\nonumber%\tag{obj}
    \max_{F_t,F_{nt}} \quad \alpha R(T) + (1-\alpha)R(U/T)
\end{equation}
\begin{equation}\tag{C1}
    \textbf{s.t.} \quad G^\tau_e \leq G_{th}  \quad \forall e \in E, \forall \tau
\end{equation}
\begin{equation}\tag{C2}
    \sum_e^E{BW}^\tau_{mid,e} \leq {BW}_{mid,th} \quad  \forall \tau
\end{equation}
\end{subequations}
where the leftmost part of the objective function is the ratio of satisfied transitional users, the rightmost part is the ratio of satisfied non-transitional users, and  $\alpha$ is the weight given to prioritize each term.  Constraints C1 and C2 are meant to limit the finite resources available to the agents at any time step  $\tau$. To solve the optimization problem, we implemented an HMARL model, deploying one agent for each EC and one for the CC. At each time step, the CC agent learns to maximize the ratio of transitional users satisfied by choosing the best split $F_t$. Conversely, each EC learns to select the split $F_{nt}$ for their coverage area that maximizes the ratio of satisfied non-transitional users utilizing the remaining resources. To exchange the information between CC and ECs, the HMARL algorithm plays out like a turn-based game, with CC acting first and ECs reacting to its decision.
%

\section{Preliminary Results}
%By implementing the system described above, we successfully trained the two policies related to the CC and the ECs. 
We trained an HMARL algorithm over the proposed architecture, training the agents' policies using the proximal policy optimization (PPO) algorithm \cite{schulman2017proximal}. To assess how the performances of our HMARL algorithm compare to the ones of static decisions for $F_t$ and $F_{nt}$, we implemented a simulation environment for the problem. For these tests, users deploy a service requiring an error rate lower than $1e-4$, with a delay threshold of $12ms$. During these preliminary tests, the constraints on ECs' GOPS and load on the midhaul link are relaxed by giving enough resources to support most of the combinations of $F_t$ and $F_{nt}$ decisions.


\input{img/satisfaction}

 Figure \ref{fig:cdf} compares the proposed HMARL solution with multiple baselines for transitional users, i.e., 1)  a random policy, 2) a static $F_t=1$, and 3) a static $F_t=3$ .
 Our proposed solution outperforms the baselines in terms of proportional satisfied users.
 Despite the close performance of functional split $F_{t}=3$ with HMARL, the latter achieves lower resource usage with the same performance, thanks to the improved policies for non-transitional users switching between $F_{nt}=5$ and $F_{nt}=6$.

While HMARL algorithm is still under optimization, we reckon that the users will always suffer some service continuity loss  due to the heuristic used for the multi-connectivity cluster composition. The latter leads to sub-optimal load distribution between O-RUs, increasing users' E2E delay and thus reducing the amount of satisfied transitional and non-transitional users.
\section{Outlook}
Preliminary results show a promising development for this work, suggesting that with proper tuning of hyperparameters (e.g. discount factor, learning rate, and entropy coefficient) higher margin of improvement with respect to static functional splits can be achieved. Additionally, a further study of multi-connectivity clustering will be conducted to solve one of the major reasons for users' reliability issues.
%Additionally, a study on different clustering techniques can lead to optimizing the load imposed by multi-connectivity which is currently one of the major reasons for users' reliability issues. 

==> sections/introduction.tex <==
\section{Introduction}\label{introduction}

 

 
Mobility management for aerial users with multi-connectivity has garnered significant attention in recent studies \cite{Bassoy2017,Hu2023}. 
With multi-connectivity, each user is simultaneously connected to and served by a cluster of distributed \glspl{ap}.
In an \gls{oran} architecture, an \gls{ec} enables the coordination among the various distributed \glspl{ap} to form the serving clusters for different users with the \gls{cca}. 
Thus user mobility is managed through dynamic reconfiguration of the serving clusters as the user moves within a \gls{cca}~\cite{Meer2024,Meer2023}.



The coordination required for multi-connectivity is enabled by a central entity connected to various distributed \glspl{ap} \cite{Hu2023}, forming a \gls{cca}.
User mobility is managed through dynamic reconfiguration of the serving clusters as the user moves \cite{Meer2024,Meer2023}.
 

During handovers between \glspl{ap}, aerial users benefiting from multi-connectivity remain connected to multiple \glspl{ap}, ensuring uninterrupted service. Handovers still take place, but the user does not incur in service disruptions. This process is hence addressed as soft handover. As a requirement for multi-connectivity, user processing needs to be centralized in a premise common to the \glspl{ap} serving them.
%However, users need their data to be processed in a premise common to the different \glspl{ap}, to achieve the needed coordination. In this work, we address the problem of enabling soft handovers for transitional users.
 For aerial users transitioning between \glspl{cca}, referred to as transitional users, being served with multi-connectivity by a cluster of \glspl{ap} is key to maintain service continuity. When the \glspl{ap} serving users belong to different \glspl{cca}, as in the case of transitional users, user processing needs to be handled in a premise common to the different \glspl{cca} involved.

We consider the \gls{oran} architecture, which supports multiple level of centralization for the handling of multi-connectivity. In this architecture, \glspl{ec}, equivalent to \gls{oran}'s O-DU, are responsible for coordinating the \glspl{ap}, \gls{oran}'s O-RUs, within their \gls{cca}. Every \gls{ec} is connected to a centralized premise, the \gls{cc}, equivalent to \gls{oran}'s O-CU, via a link called midhaul, as illustrated in \autoref{fig:hcran}. In order centralize users' processing where needed, enabling multi-connectivity and soft handovers, we consider the functional split paradigm.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{img/hcran_architecture2.pdf}
    \caption{\gls{oran} architecture considered.}
    \label{fig:hcran}
\end{figure}





In \gls{oran} networks, the processing of user data is composed of a chain of functions. Thanks to virtualization, the function chain can be deployed anywhere in the network, regardless of specific premises. \gls{fs} allows the function chain to be split in one point, effectively deploying some of the functions in \glspl{ec} and the rest in \gls{cc}.
This can be leveraged to centralize the \glspl{pf} of transitional users within the \gls{cc}, allowing them to be continuously served through multi-connectivity while soft handovers are executed. 
Non-transitional users do not require this level of centralization, as the \gls{ec} serving them can act as the centralization point for multi-connectivity. 
Moreover, \gls{fs} influence the delay perceived by users: a more distributed \glspl{pf} setup results in lower user-perceived delay, and vice versa. 
This consideration is critical when deploying services with strict latency requirements.
Depending on the \gls{fs}, the amount of network resources necessary to deploy the \glspl{pf} varies as well: the more \glspl{pf} are executed at \glspl{ec}' premises, the more computational resources at \glspl{ec} are needed. On the other hand, the less \glspl{pf} are processed on the \glspl{ec}, the more data needs to be transported to the \gls{cc}, imposing a higher traffic on the midhaul link, the link between \glspl{ec} and the \gls{cc}. 
\autoref{fig:split} presents the chain of \glspl{pf} considered considered in this paper, as well as the tradeoff between \gls{GOPS} required at \glspl{ec} and the bandwidth required on the midhaul link to support them.
 

%%para 4th 
%short para about the problem
%A functional split is traditionally deployed statically for the whole infrastructure. However, by deploying a functional split suitable for transitional users' soft handovers, non-transitional users in the network would be negatively affected due to the high level of centralization. Additionally, in infrastructures with constrained resources, functional split configuration may require more resources than there are avaiable.
Traditionally, a static \gls{fs} is deployed across the entire network. However, deploying splits optimized for transitional users' soft handovers can negatively impact non-transitional users: due to the higher centralization of \glspl{pf} the delay perceived throughout the network is increased. On the other hand, deploying splits optimized for non-transitional users would have transitional users unable to use multi-connectivity, disruption their service continuity. Moreover, the resources requested by a certain \gls{fs} for \glspl{pf} execution scale with the amount of users to serve. In a network yielding constrained computational capabilities, it is paramount to find a split that can support users with the available resources, accounting for unexpected loads, while complying with users' requirements. Clearly, such split can not be easily defined: a split that can be deemed optimal for a certain scenario may not be as optimal later in time.


%para 5th
%AI particularly HMARL as the solution to the above problem
A novel approach to addressing these challenges is the flexible \gls{fs} paradigm. Using flexible \gls{fs}, the deployment of \glspl{pf} can be dynamically adjusted to align with available resources and users' constraints. Additionally, by deploying distinct flexible functional split configurations for transitional and non-transitional users, each group can be managed more efficiently thanks to tailored \glspl{fs}. The choice of \glspl{fs} for the different user groups can be considered a dynamic resource allocation problem. While optimal solvers could address this problem on a small scale, the dynamic nature and complexity of the \gls{oran} environment make their use challenging. Conversely, literature shows promising results on the usage of \glspl{drl} dynamic resource allocation problems of this scale.
 In this context, the proposed solution utilizes a \gls{hmarl} algorithm, enabling fine-grained control over functional split configurations of each user group while considering resource consumption and users' service constraints.
 
%In this work, we introduce a novel approach by embedding message passing within the \gls{hmarl} algorithm, offering a more realistic alternative to the assumption that all \glspl{ec} have full knowledge of resource availability. High-level agents communicate midhaul load information to lower-level agents in a publish-subscribe manner, enabling dynamic, resource-aware adjustments based on current conditions, without requiring global knowledge across the network
The contribution of this work are:
\begin{itemize}
    \item We formulate an optimization problem aimed at ensuring service continuity for all users in the network. This involves identifying flexible functional split configurations to meet user service requirements, support soft handovers, and optimize the use of limited network resources.
    \item We propose a \gls{hmarl} algorithm to solve our optimization problem. Here, a high-level agent focuses on enabling soft handovers for transitional users, while multiple low-level agents maximize performances of non-transitional users in their \gls{cca}.
    \item We introduce a novel communication mechanism within \gls{hmarl}, where high-level and low-level agents interact in a turn-based manner, simulating the message-passing process of a distributed system.
    \item Finally, we test the \gls{hmarl} algorithm against industry-standard functional split configurations to validate the effectiveness of our approach.
\end{itemize}


 %remainder
 % The remainder of this paper is organized as  follows.  In Section~\ref{rw}, related works in the literature are presented. In Section~\ref{modelling}, the system model with a problem formulation are provided. In Section~\ref{impl}, our implementation of the HMARL algorithm is presented with a comparison study. Finally, Section~\ref{outlook} sums up the conclusions of this paper, as well as the future research directions.







% Millions of Unmanned Aerial Devices (UAVs) are expected to be deployed in the existing 5G and beyond infrastructures. These can fulfill many tasks, among which are services such as outage management, healthcare, goods transportation security and public safety \cite{hossein_motlagh_low-altitude_2016}. A good part of these services require UAVs (and aerial users alike) to maintain low-latency and highly reliable communications to implement tele-operated driving, video streaming and collision avoidance systems \cite{yoshizawa_overview_2019}. 
% Such services can present strict requirements, with delay limits that can range between $1ms$ and tens of milliseconds, and a maximum error rate that can go from $10^{-3}$ and lower.

% Although compliance with such services' requirements is complex per se, challenges arise when coming to roaming mobile hosts. When the latter needs to move from the coverage area of an access point to another, a handover takes place, requiring the breaking of the existing connection and the creation of a new one with the new access point, disconnecting the user from the infrastructure for  $10ms$ to $12.5ms$ \cite{3gpp_lte_nodate}. Clearly, incurring in such delays and disconnections prevents the hosts from complying with their strict service requirements. For this reason, multi-connectivity technologies such as Joint Transmission (JT) \cite{bassoy_coordinated_2017} have been exploited in literature to sensibly reduce the amount of handovers to perform. Thanks to JT, a cluster of  different access points serves a single user ensuring that, during handovers between single base stations, the user is still served by the remaining members of the cluster, thus avoiding service disruptions. The latter process takes the name of soft-handover. 

% However, in order to enable multi-connectivity, orchestration and scheduling for the communication between antennas and users have to be centralized in the infrastructure. In this study, we consider an ORAN architecture composed by a hierarchy of computing premises. Figure \ref{fig:hcran} presents the ORAN infrastructure and the different layers that compose it: \textit{i)} Central Cloud (CC), \textit{ii)} Edge Clouds (ECs), \textit{iii)} Base Stations (BSs). The CC is a centralized computation premise situated in the cloud. The latter is connected to the ECs via a shared link called midhaul link. ECs are computing premises situated closer to the users, and perform the data processing for a set of BSs and users: specifically the ones in their Cloud Coverage Area (CCA). While ECs can be used as centralization point to enable JT for users roaming inside a CCA, users transitioning from one CCA to another are inevitably served by BSs belonging to different CCAs, needing their processing to be executed at the CC, the closest centralization point in the infrastructure. Intuitively, when the transition to a new CCA is completed, the new CCA's EC can be used as the new centralization point.


% Such data processing relocation can be achieved thanks to functional split: by splitting the chain of functions needed for data processing, it is possible to deploy part of it in the ECs and the remaining functions at the CC. 
% By doing so, we can vary the centralization level of users, enabling them to benefit from JT during both intra-CCA and inter-CCA roaming. 
% Functional split affects importantly the infrastructure's resources such as computation resources at ECs and the bandwidth load on the midhaul link, as seen in Figure \ref{fig:split}. Additionally, functional split directly affects users in the network: by moving the computation of their functions further in the cloud, the end-to-end latency perceived by the latter increases significantly, making it harder to comply with their service requirements. For this reason, users performing inter-CCA crossing (from now own called transitional users) have to be  carefully addressed, since most of their processing functions are executed at CC's premises due to JT requirements. At the same time, applying functional splits enabling soft handovers for transitional users to the whole network can lead to sub-optimal resources allocation, impacting all users' performances. While functional split is traditionally configured statically for the entire network, literature suggests that, when dynamic dimensions are added to a scenario (e.g.  time, changing load or resources, etc.), it can beneficial to dynamically updated the functional split configuration \cite{alba_dynamic_2022}. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/split.pdf}
    \caption{\gls{fs} and resulting resources tradeoff.}
    \label{fig:split}
\end{figure}

% In this paper, we want to exploit the flexible functional split paradigm in order to address user's service continuity. In particular, we focus on implementing soft handovers for transitional users, since they are particularly difficult and resource-intensive to handle, while handling the rest of the users as optimally as possible with the remaining resources. To do so, we deploy a Hierarchical Multi-Agent Reinforcement Learning (HMARL) algorithm, able to understand the resources usage and deploying optimal functional split configurations to help users avoiding service disruptions. The remainders of this paper are the following: in Section~\ref{rw} contributions on the topic found in the literature are presented, in Section~\ref{modelling} the modelling of the problem is given, in Section~\ref{impl} our implementation for the HMARL algorithm is presented, as well as the comparison with industry standard methods. Finally, Section~\ref{outlook} sums up the conclusions of this work, as well as presenting the future directions envisioned for this work.




 




